Task Scheduling for Efficient Inference of Large Language Models on Single Moderate GPU Systems

Large language models~(LLMs) are known for their high demand on computing resources and memory due to their substantial model size, which leads to inefficient inference on moderate GPU systems. Techniques like quantization or pruning can shrink model sizes but often impair accuracy, making them unsuitable for practical applications. In this work, we introduce \modelname{}, a high-performance inference engine designed to speed up LLM inference without compromising model accuracy. \modelname{} incorporates three innovative methods to increase inference efficiency: 1) model partitioning to allow asynchronous processing of tasks across CPU computation, GPU computation, and CPU-GPU communication, 2) an adaptive partition algorithm to optimize the use of CPU, GPU, and PCIe communication capabilities, and 3) a token assignment strategy to handle diverse prompt and generation tasks during LLM inference. Comprehensive experiments were conducted with various LLMs such as Mixtral, LLaMA-2, Qwen, and PhiMoE across three test environments featuring different CPUs and GPUs. The experimental findings demonstrate that \modelname{} achieves speeds between $1.11\times$ to $1.80\times$ faster in decoding and $1.69\times$ to $6.33\times$ faster in pre-filling, leading to an overall speedup ranging from $1.25\times$ to $2.04\times$ compared to state-of-the-art solutions, llama.cpp and Fiddler.

==> 3motivation.tex <==

\section{Motivation}
\subsection{Insufficient utilization of limited resource.}
In consumer-grad computers, the GPU memory and the CPU computation resource are constrained. Fully leveraging those available resources to enhance inference performance presents a significant challenge. Prior studies typically exploit just one type of resource at a time. For instance, Fiddle relies solely on CPU resources for MLP computations and solely on GPU resources for other Non-MoE layers. Llama-cpp partitions model layers into those processed on the CPU and those on the GPU. Mixtral-offloading involves loading expert weights onto the GPU for computation. However, none of these approaches simultaneously exploit multiple resources, leading to inefficiencies. Consequently, our approach aims to concurrently perform CPU and GPU computations, along with efficient communication between the two, to maximize resource usage and minimize operational overhead. To accomplish this goal, we propose dividing the weight tensor into three segments: 1) stored in CPU memory and processed on the CPU (\ccname{}), 2) stored in GPU memory and processed on the GPU (GG), and 3) stored in CPU memory and processed on the GPU (CG). Similarly to tensor parallelism, we can run three separate components concurrently and then merge their results once all processes are completed.

\subsection{Determining the slicing rate of each part.}
The overhead of CPU computation, GPU computation and communication between CPU and GPU are different from each other. The best slicing rate for each part will depend heavily on the performance model of these operations. What's more, slicing rates of each part also affect the final time cost a lot. Manually determining the silcing rate is a simple solution. However, it is not intelligent to manually test various combinations of slicing rates to find the best one. Therefore, a method to automatically determine the slicing rate of each part is required.

Two primary challenges exist in determining the slicing rate. Firstly, it involves creating a performance model for each operation and formulating the optimization problem. Secondly, the slicing rate for GG is intricately linked to the constraints of GPU memory, complicating the optimization process when other slicing rates are involved.
\subsection{Different slicing rates between prompt and generation phase.}
It is obvious that the best slicing rate differs between the prompt and generation phases. What's more, the best slicing rate in prompt phase will result in poor performance in the generation phase and verse visa. However, switching the slicing rate from the best one in the prompt phase to that in the generation phase requires expensive model weight transferring. Consequently, we propose to subdivide tokens into two categories during the prompt phase: (1) those executed with the slicing rate produced during the generation phase and (2) those executed with the zero slicing rate of \ccname{}. In this way, we can compensate for the differential slicing rates across the two stages.


